Energy as a source of pre-service teachers' conceptions about radioactivity

Although researchers have extensively studied student conceptions of radioactivity, the conceptions held by pre-service teachers on this subject are largely absent from the literature. We conducted a qualitative content analysis of problem-centered interviews with pre-service teachers N = 13 to establish which conceptions are held by pre-service teachers and to examine these conceptions' structure in coordination classes. As has already been observed in students, some pre-service teachers inadequately differentiate between radioactive matter and ionizing radiation and between fission and decay. We also observed that pre-service teachers tend to describe the activation of materials due to ionizing radiation despite having previously denied an activation, thus showing that the conception of activation of materials can reemerge in particular framings. Within the interviews conducted, the concept of energy emerged as a central coordination class regarding radioactivity. This coordination class appeared across contexts and proved fruitful in explaining pre-service teachers' conceptions about radioactivity. We will use the results from this study to develop a teaching-learning laboratory for pre-service teachers in which they can actively study high school students' conceptions while reflecting on their own. In this way, these findings will contribute to improving the structure of nuclear physics courses at the university.

==> Bibitems.tex <==
\bibitem{Pham.2012}Pham, G., Koch, T., Helmke, A., Schrader, F., Helmke, T. \& Eid, M. Do Teachers Know How Their Teaching is Perceived by their Pupils?. {\em Procedia - Social And Behavioral Sciences}. \textbf{46} pp. 3368-3374 (2012)
\bibitem{Pinto.2007}Pintó, R. \& Couso, D. Contributions from Science Education Research. (Springer,2007), http://site.ebrary.com/lib/alltitles/docDetail.action?docID=10205286
\bibitem{Plotz.2019}Plotz, T. \& Hollenthoner, F. Replicating a study about children's drawings concerning radiation. {\em Multidisciplinary Journal For Education, Social And Technological Sciences}. \textbf{6}, 71 (2019)
\bibitem{Plotz.2019b}Plotz, T. \& Hollenthoner, F. Replicating a study about children's drawings concerning radiation. {\em Multidisciplinary Journal For Education, Social And Technological Sciences}. \textbf{6}, 71 (2019)
\bibitem{Plotz.2017}Plotz, T. Lernprozesse zu nicht-sichtbarer Strahlung. (Logos Verlag Berlin GmbH,2017)
\bibitem{Plotz.2017b}Plotz, T. Students&apos; Conceptions of Radiation and What to Do about Them. {\em Physics Education}. \textbf{52}, Artikel 014004 (6 Seiten) (2017), http://dx.doi.org/10.1088/1361-6552/52/1/014004
\bibitem{Plotz.2021}Plotz, T. \& Fitzgerald, B. Superheroes of the Electromagnetic Spectrum: A Non-Traditional Way of Teaching Ionising Radiation. {\em Eurasia Journal Of Mathematics, Science And Technology Education}. \textbf{17}, em1975 (2021)
\bibitem{Petri.1998}Petri, J. \& Niedderer*, H. A learning pathway in high–school level quantum atomic physics. {\em International Journal Of Science Education}. \textbf{20}, 1075-1088 (1998)
\bibitem{Plotz.2016}Plotz, T. \& Hopf, M. Two concepts of radiation - a case study investigating existing preconceptions. {\em European Journal Of Science And Mathematics Education}. \textbf{4}, 447-459 (2016)
\bibitem{Posner.1982}Posner, G., Strike, K., Hewson, P. \& Gertzog, W. Accommodation of a scientific conception: Toward a theory of conceptual change. {\em Science Education}. \textbf{66}, 211-227 (1982)
\bibitem{Posner.1982b}Posner, G. \& Und weitere Accommodation of a Scientific Conception: Toward a Theory of Conceptual Change. {\em Science Education}. \textbf{66}, 211-227 (1982)
\bibitem{Prather.2005}Prather, E. Students' Beliefs About the Role of Atoms in Radioactive Decay and Half-life. {\em Journal Of Geoscience Education}. \textbf{53}, 345-354 (2005)
\bibitem{Radiker.2019}Rädiker, S. \& Kuchartz, U. Analyse qualitativer Daten mit MAXQDA: Text, Audio und Video. (Springer VS,2019)
\bibitem{Redfors.2001}Redfors, A. \& Ryder, J. University physics students' use of models in explanations of phenomena involving interaction between metals and electromagnetic radiation. {\em International Journal Of Science Education}. \textbf{23}, 1283-1301 (2001)
\bibitem{Reed.2011}Reed, B. The Physics of the Manhattan Project. (Springer Berlin Heidelberg,2011)
\bibitem{Rego.2006}Rego, F. \& Peralta, L. Portuguese students' knowledge of radiation physics. {\em Physics Education}. \textbf{41}, 259-262 (2006)
\bibitem{Posner.1982c}Posner, G. \& Others, A. Accommodation of a Scientific Conception: Toward a Theory of Conceptual Change. {\em Science Education}. \textbf{66}, 211-227 (1982)
\bibitem{Lave.1991}Lave, J. Situating learning in communities of practice. {\em Perspectives On Socially Shared Cognition}. pp. 63-82 (1991)
\bibitem{Leone.2018}Leone, M., Robotti, N. \& Verna, G. `Rutherford's experiment' on alpha particles scattering: the experiment that never was. {\em Physics Education}. \textbf{53}, 035003 (2018)
\bibitem{Levin.2009}Levin, D., Hammer, D. \& Coffey, J. Novice Teachers' Attention to Student Thinking. {\em Journal Of Teacher Education}. \textbf{60}, 142-154 (2009)
\bibitem{Lijnse.1990}Lijnse, P., Eijkelhof, H., Klaassen, C. \& Scholte, R. Pupils' and mass–media ideas about radioactivity. {\em International Journal Of Science Education}. \textbf{12}, 67-78 (1990)
\bibitem{Loughran.2007}Loughran, J., Berry, A. \& Mulhall, P. Pedagogical Content Knowledge: What Does it Mean to Science Teachers?. {\em Contributions From Science Education Research}. pp. 93-105 (2007)
\bibitem{Mayring.2015}Mayring, P. Qualitative Inhaltsanalyse: Grundlagen und Techniken. (Beltz,2015), http://www.beltz.de/fileadmin/beltz/leseproben/978-3-407-25730-7.pdf
\bibitem{Millar.1989}Millar, R. Constructive criticisms. {\em International Journal Of Science Education}. \textbf{11}, 587-596 (1989)
\bibitem{Millar.1996}Millar, R. \& Gill, J. School students' understanding of processes involving radioactive substances and ionizing radiation. {\em Physics Education}. \textbf{31}, 27-33 (1996)
\bibitem{Millar.1990}Millar, R., Klaassen, K. \& Eijkelhof, H. Teaching about radioactivity and ionising radiation: An alternative approach. {\em Physics Education}. \textbf{25}, 338-342 (1990)
\bibitem{MoralesLopez.2022}Morales López, A. \& Tuzón Marco, P. Misconceptions, Knowledge, and Attitudes Towards the Phenomenon of Radioactivity. {\em Science & Education}. \textbf{31}, 405-426 (2022)
\bibitem{Murphy.2006}Murphy, P., Lunn, S. \& Jones, H. The impact of authentic learning on students' engagement with physics. {\em The Curriculum Journal}. \textbf{17}, 229-246 (2006)
\bibitem{Neumann.2011}Neumann, S. \& Hopf, M. Was verbinden Schülerinnen und Schüler mit dem Begriff "Strahlung"? Paralleltitel: What do students associate with the German Term "Strahlung" (=radiation)?. {\em Zeitschrift Für Didaktik Der Naturwissenschaften}. \textbf{17} pp. 157-176; 1,2 MB (2011), http://archiv.ipn.uni-kiel.de/zfdn/pdf/17_Neumann.pdf
\bibitem{Neumann.2012}Neumann, S. \& Hopf, M. Students' Conceptions About `Radiation': Results from an Explorative Interview Study of 9th Grade Students. {\em Journal Of Science Education And Technology}. \textbf{21}, 826-834 (2012)
\bibitem{Neumann.2013}Neumann, S. \& Hopf, M. Children's Drawings About “Radiation”—Before and After Fukushima. {\em Research In Science Education}. \textbf{43}, 1535-1549 (2013)
\bibitem{Neumann.2013b}Neumann, S. \& Hopf, M. Students' Ideas About Nuclear Radiation – Before and After Fukushima. {\em EURASIA Journal Of Mathematics, Science And Technology Education}. \textbf{9} (2013)
\bibitem{Niedderer.2007}Niedderer, H., Budde, M., Givry, D., Psillos, D. \& Tiberghien, A. Learning Process Studies. {\em Contributions From Science Education Research}. pp. 159-171 (2007)
\bibitem{Niedderer.1992}Niedderer, H. \& Schecker, H. Towards an explicit description of cognitive systems for research in physics learning.  (1992)
\bibitem{Rieder.1992}Rieder, W. Eine elementare Herleitung der Rutherford-Streuung. {\em Der Mathematische Und Naturwissenschaftliche Unterricht}. \textbf{45}, 304-305 (1992)
\bibitem{Treagust.2008}Treagust, D. Connecting Theory and Practice: Towards a Broader Understanding of Conceptual Change in Science. {\em Four Decades Of Research In Science Education-from Curriculum Development To Quality Improvement: From Curriculum Development To Quality Improvement}. pp. 101 (2008)
\bibitem{Trumper.1996}Trumper, R. \& Gorsky, P. A cross-college age study about physics students' conceptions of force in pre-service training for high school teachers. {\em Physics Education}. \textbf{31}, 227-236 (1996), https://iopscience.iop.org/article/10.1088/0031-9120/31/4/021
\bibitem{Tsaparlis.2013}Tsaparlis, G., Hartzavalos, S. \& Nakiboğlu, C. Students' Knowledge of Nuclear Science and Its Connection with Civic Scientific Literacy in Two European Contexts: The Case of Newspaper Articles. {\em Science & Education}. \textbf{22}, 1963-1991 (2013)
\bibitem{Tuniz.2012}Tuniz, C. Radioactivity: A very short introduction. (Oxford Univ. Press,2012)
\bibitem{vandeBogart.29.07.201530.07.2015}Van de Bogart, K., Dounas-Frazer, D., Lewandowski, H. \& Stetzer, M. The Role of Metacognition in Troubleshooting: An Example From Electronics. {\em 2015 Physics Education Research Conference Proceedings}. pp. 339-342
\bibitem{vanDijk.2007}Van Dijk, E. \& Kattmann, U. A research model for the study of science teachers' PCK and improving teacher education. {\em Teaching And Teacher Education}. \textbf{23}, 885-897 (2007)
\bibitem{Wagner.2010}Wagner, J. \& Cadet, J. Oxidation reactions of cytosine DNA components by hydroxyl radical and one-electron oxidants in aerated aqueous solutions. {\em Accounts Of Chemical Research}. \textbf{43}, 564-571 (2010)
\bibitem{Willers.2004}Willers, H., Dahm-Daphi, J. \& Powell, S. Repair of radiation damage to DNA. {\em British Journal Of Cancer}. \textbf{90}, 1297-1301 (2004), https://www.nature.com/articles/6601729#change-history
\bibitem{Witzel.1985}Witzel, A. Das problemzentrierte Interview. {\em Qualitative Forschung In Der Psychologie : Grundfragen, Verfahrensweisen, Anwendungsfelder}. pp. 227-255 (1985)
\bibitem{Woithe.2017}Woithe, J., Wiener, G. \& Van der Veken, F. Let's have a coffee with the Standard Model of particle physics!. {\em Physics Education}. \textbf{52}, 034001 (2017), https://iopscience.iop.org/article/10.1088/1361-6552/aa5b25
\bibitem{Wood.2014}Wood, A., Galloway, R., Hardy, J. \& Sinclair, C. Analyzing learning during Peer Instruction dialogues: A resource activation framework. {\em Physical Review Special Topics - Physics Education Research}. \textbf{10} (2014)
\bibitem{YalcnkayaOnder.2020}Yalçınkaya Önder, E. \& Pekmez, E. Argumentation Practice in the Context of Nuclear Power Plants. {\em Mediterranean Journal Of Educational Research}. \textbf{14}, 116-135 (2020)
\bibitem{Yerushalmi.2006}Yerushalmi, E. \& Polingher, C. Guiding students to learn from mistakes. {\em Physics Education}. \textbf{41}, 532-538 (2006)
\bibitem{Thomas.1998}Thomas, P. \& Schwenz, R. College physical chemistry students' conceptions of equilibrium and fundamental thermodynamics. {\em Journal Of Research In Science Teaching}. \textbf{35}, 1151-1160 (1998)
\bibitem{Riesch.1975}Riesch, W. \& Westphal, W. Modellhafte Schülervorstellungen zur Ausbreitung radioaktiver Strahlung. {\em Der Physikunterricht}. \textbf{1975/4} pp. 75-85 (1975)
\bibitem{Rutherford.1911}Rutherford, E. LXXIX. The scattering of \textgreeka and \textgreekb particles by matter and the structure of the atom. {\em The London, Edinburgh, And Dublin Philosophical Magazine And Journal Of Science}. \textbf{21}, 669-688 (1911)
\bibitem{Rutherford.1909}Rutherford, E. \& Royds, T. XXI. The nature of the \textgreeka particle from radioactive substances. {\em The London, Edinburgh, And Dublin Philosophical Magazine And Journal Of Science}. \textbf{17}, 281-286 (1909)
\bibitem{Siler.2013}Siler, S., Klahr, D. \& Bryan Matlen Conceptual change when learning experimental design. {\em International Handbook Of Research On Conceptual Change}. pp. 150-170 (2013)
\bibitem{Simon.2019}Simon, F. Der Einfluss von Betreuung und Betreuenden auf die Wirksamkeit von Schülerlaborbesuchen: Eine Zusammenhangsanalyse von Betreuungsqualität, Betreuermerkmalen und Schülerlaborzielen sowie Replikationsstudie zur Wirksamkeit von Schülerlaborbesuchen. (Logos Verlag Berlin,2019), https://directory.doabooks.org/handle/20.500.12854/64421
\bibitem{Slotta.2011}Slotta, J. In Defense of Chi's Ontological Incompatibility Hypothesis. {\em Journal Of The Learning Sciences}. \textbf{20}, 151-162 (2011)
\bibitem{SODDY.1913}SODDY, F. The Radio-Elements and the Periodic Law. {\em Nature}. \textbf{91}, 57-58 (1913)
\bibitem{Steel.1996}Steel, G. From targets to genes: a brief history of radiosensitivity. {\em Physics In Medicine And Biology}. \textbf{41}, 205-222 (1996)
\bibitem{TamerG.Amin.2014}Tamer G. Amin, Carol L. Smith \& Marianne Wiser Student Conceptions and Conceptual Change. {\em Handbook Of Research On Science Education}. (2014), https://www.routledgehandbooks.com/doi/10.4324/9780203097267.ch4
\bibitem{Chi.2005}Chi, M. Commonsense Conceptions of Emergent Processes: Why Some Misconceptions Are Robust. {\em Journal Of The Learning Sciences}. \textbf{14}, 161-199 (2005)
\bibitem{Chi.2013}Chi, M. Two Kinds and Four Sub-Types of Misconceived Knowledge, Ways to Change it, and the Learning Outcomes. {\em International Handbook Of Research On Conceptual Change}. (2013)
\bibitem{Choppin.2013}Choppin, G., Ekberg, C., Liljenzin, J. \& Rydberg, J. Radiochemistry and nuclear chemistry. (Academic Press,2013), http://www.sciencedirect.com/science/book/9780124058972
\bibitem{Colclough.2011}Colclough, N., Lock, R. \& Soares, A. Pre–service Teachers' Subject Knowledge of and Attitudes about Radioactivity and Ionising Radiation. {\em International Journal Of Science Education}. \textbf{33}, 423-446 (2011)
\bibitem{Cooper.2003}Cooper, S., Yeo, S. \& Zadnik, M. Australian students' views on nuclear issues: Does teaching alter prior beliefs?. {\em Physics Education}. \textbf{38}, 123-129 (2003)
\bibitem{DavidHammer.2003}David Hammer \& Andrew Elby Tapping Epistemological Resources for Learning Physics. {\em Journal Of The Learning Sciences}. \textbf{12}, 53-90 (2003)
\bibitem{Boyes.1994}Boyes, E. \& Stanisstreet, M. Children's Ideas about Radioactivity and Radiation: sources, mode of travel, uses and dangers. {\em Research In Science & Technological Education}. \textbf{12}, 145-160 (1994)
\bibitem{DavidHammer.2004}David Hammer, Andrew Elby, Rachel E. Scherr \& Edward F. Redish Resources , framing , and transfer.  (2004)
\bibitem{DiLisi.2018}DiLisi, G., Hirsch, A., Murray, M. \& Rarick, R. Thorium and Molten Salt Reactors: Essential Questions for Classroom Discussions. {\em The Physics Teacher}. \textbf{56} pp. 253-257 (2018)
\bibitem{diSessa.1993}DiSessa, A. Toward an Epistemology of Physics. {\em Cognition And Instruction}. \textbf{10}, 105-225 (1993)
\bibitem{diSessa.2013}DiSessa, A. A Bird's-Eye View of the “Pieces” vs. “Coherence” Controversy (from the “Pieces” side of the Fence). {\em International Handbook Of Research On Conceptual Change}. (2013)
\bibitem{Disessa.2008}Disessa, A. A bird's-eye view of the "pieces" vs. "coherence" controversy (from the "pieces" side of the fence). {\em International Handbook Of Research On Conceptual Change}. pp. 35-60 (2008)
\bibitem{Dianovsky.2013}Dianovsky, M., Chinn, C., Duncan, R. \& Rinehart, R. Promoting Conceptual Change Through Inquiry.  (2013)
\bibitem{Bohr.1939}Bohr, N. \& Wheeler, J. The Mechanism of Nuclear Fission. {\em Physical Review}. \textbf{56}, 426-450 (1939), http://link.aps.org/pdf/10.1103/PhysRev.56.426
\bibitem{AcarSesen.2010}Acar Sesen, B. \& Ince, E. Internet as a source of misconception: "Radiation and radioactivity". {\em Turkish Online Journal Of Educational Technology}. \textbf{9} pp. 94-100 (2010)
\bibitem{Alsop.2001}Alsop, S. Living with and learning about radioactivity: A comparative conceptual study. {\em International Journal Of Science Education}. \textbf{23}, 263-281 (2001)
\bibitem{Henriksen.1996}Henriksen, E. Laypeople's Understanding of Radioactivity and Radiation. {\em Radiation Protection Dosimetry}. \textbf{68}, 191-196 (1996)
\bibitem{Henriksen.2001}Henriksen, E. \& Jorde, D. High school students' understanding of radiation and the environment: Can museums play a role?. {\em Science Education}. \textbf{85}, 189-206 (2001)
\bibitem{Hoehn.2018}Hoehn, J. \& Finkelstein, N. Students' flexible use of ontologies and the value of tentative reasoning: Examples of conceptual understanding in three canonical topics of quantum mechanics. {\em Physical Review Physics Education Research}. \textbf{14} (2018)
\bibitem{Hoehn.2018b}Hoehn, J., Gifford, J. \& Finkelstein, N. Dynamics of students' ontological reasoning across contexts in modern physics. {\em 2018 Physics Education Research Conference Proceedings}. (2018), https://www.compadre.org/per/items/detail.cfm?ID=14798
\bibitem{Hoehn.2019}Hoehn, J., Gifford, J. \& Finkelstein, N. Investigating the dynamics of ontological reasoning across contexts in quantum physics. {\em Physical Review Physics Education Research}. \textbf{15} (2019)
\bibitem{Hon.2013}Hon, G. \& Goldstein, B. J. J. Thomson's plum-pudding atomic model: The making of a scientific myth. {\em Annalen Der Physik}. \textbf{525}, A129-A133 (2013)
\bibitem{Hull.2020}Hull, M. \& Hopf, M. Student understanding of emergent aspects of radioactivity. {\em International Journal Of Physics & Chemistry Education}. \textbf{12}, 19-33 (2020), https://ijpce.org/index.php/IJPCE/article/view/125
\bibitem{Hull.2021}Hull, M., Jansky, A. \& Hopf, M. Probability-related naïve ideas across physics topics. {\em Studies In Science Education}. \textbf{57}, 45-83 (2021)
\bibitem{Jansky.2019}Jansky, A. Die Rolle von Schülervorstellungen zu Wahrscheinlichkeit und Zufall im naturwissenschaftlichen Kontext : Konzeption und Evaluation einer Lehr-Lern-Einheit zur Wahrscheinlichkeitstheorie in der Radioaktivität.  (2019)
\bibitem{JuliaWoithe.2017}Julia Woithe, Gerfried J Wiener \& Frederik F Van der Veken Let's have a coffee with the Standard Model of particle physics!. {\em Physics Education}. \textbf{52}, 034001 (2017)
\bibitem{Klaassen.1990}Klaassen, K. Considering an alternative approach to teaching radioactivity.  (1990)
\bibitem{Kontomaris.2020}Kontomaris, S., Malamou, A., Balogiannis, G. \& Antonopoulou, N. A simplified approach for presenting the differences between ionising and non-ionising electromagnetic radiation. {\em Physics Education}. \textbf{55}, 025007 (2020)
\bibitem{Eijkelhof.1990}Eijkelhof, H. Radiation and risk in physics education: Straling en risico's in het natuurkundeonderwijs: Zugl.: Utrecht, Univ., Diss. : 1990. (CD-Beta Press,1990)
\bibitem{Fajans.1919}Fajans, K. Radioaktivität und Die Neueste Entwickelung der Lehre Von Den Chemischen Elementen. (Springer Vieweg. in Springer Fachmedien Wiesbaden GmbH,1919)
\bibitem{Gropengieer.2016}Gropengießer, H. Kattmann, U. (2015). Schüler besser verstehen. Alltagsvorstellungen im Biologieunterricht. {\em Zeitschrift Für Didaktik Der Naturwissenschaften}. \textbf{22}, 231-232 (2016)
\bibitem{Gupta.2010}Gupta, A., Hammer, D. \& Redish, E. The Case for Dynamic Models of Learners' Ontologies in Physics. {\em Journal Of The Learning Sciences}. \textbf{19}, 285-321 (2010)
\bibitem{Hammer.1996}Hammer, D. More than misconceptions: Multiple perspectives on student knowledge and reasoning, and an appropriate role for education research. {\em American Journal Of Physics}. \textbf{64}, 1316-1325 (1996)
\bibitem{Hammer.2011}Hammer, D., Gupta, A. \& Redish, E. On Static and Dynamic Intuitive Ontologies. {\em Journal Of The Learning Sciences}. \textbf{20}, 163-168 (2011)
\bibitem{Hattie.2009}Hattie, J. Visible learning: A synthesis of over 800 meta-analyses relating to achievement. (Routledge,2009)
\bibitem{Hayes.1960}Hayes, R. \& Butler, W. Growth and decay of radionuclides: A demonstration. {\em Journal Of Chemical Education}. \textbf{37}, 590 (1960)
\bibitem{Zwickl.2014}Zwickl, B., Finkelstein, N. \& Lewandowski, H. Incorporating learning goals about modeling into an upper-division physics laboratory experiment. {\em American Journal Of Physics}. \textbf{82}, 876-882 (2014)

